Architecture-Agnostic Masked Image Modeling -- From ViT back to CNN

Masked image modeling, an emerging self-supervised pre-training method, has shown impressive success across numerous downstream vision tasks with Vision transformers. Its underlying idea is simple: a portion of the input image is masked out and then reconstructed via a pre-text task. However, the working principle behind MIM is not well explained, and previous studies insist that MIM primarily works for the Transformer family but is incompatible with CNNs. In this work, we observe that MIM essentially teaches the model to learn better middle-order interactions among patches for more generalized feature extraction. We then propose an Architecture-Agnostic Masked Image Modeling framework (A$^2$MIM), which is compatible with both Transformers and CNNs in a unified way. Extensive experiments on popular benchmarks show that A$^2$MIM learns better representations without explicit design and endows the backbone model with the stronger capability to transfer to various downstream tasks.

==> tables/tab_ablation_comparison.tex <==
\begin{table}[H]
    \setlength{\tabcolsep}{1.3mm}
    \centering
    \caption{Comparison of A$^2$MIM with advanced components to current state-of-the-art methods on ImageNet-1K.}
    % \vspace{-0.5em}
    \label{tab:ablation_comp}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
    Module                & ResNet-50 & ViT-B     \\
                          & FT (A3)   & FT        \\ \hline
    A$^2$MIM              & 78.8      & 84.2      \\
    A$^2$MIM+MLP (DW)     & 78.9      & 84.3      \\
    A$^2$MIM+MLP (DW)+HoG & \bf{79.0} & \bf{84.6} \\ \hline
    BYOL                  & 78.9      & -         \\
    MoCo.V3               & \bf{79.0} & 83.2      \\
    MaskFeat              & -         & 84.0      \\
    PeCo                  & -         & 84.5      \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/tab_ablation_component.tex <==
\begin{table}[H]
    \setlength{\tabcolsep}{1.3mm}
    \centering
    \caption{Ablation of the decoder structures and the prediction targets on ImageNet-1K.}
    % \vspace{-0.5em}
    \label{tab:ablation_advanced}
\resizebox{\linewidth}{!}{
    \begin{tabular}{cc|cc}
    \toprule
            & Module                      & ResNet-50 & ViT-B     \\ \hline
            & Linear                      & 78.8      & 82.4      \\
            & 2-layer MLP                 & 78.8      & 82.4      \\
    Decoder & 2-layer MLP (w/ DW)         & 78.8      & 82.5      \\
            & 2-layer Transformer         & 78.6      & 82.3      \\
            & 2-layer Transformer (w/ DW) & \bf{78.9} & \bf{82.6} \\ \hline
            & RGB                         & 78.8      & 82.4      \\
    Target  & HoG Feature                 & 78.9      & 82.6      \\
            & DINO Feature                & \bf{78.9} & \bf{82.7} \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/tab_ablation_in1k.tex <==
\begin{table}[H]
    \setlength{\tabcolsep}{1.3mm}
    \centering
    \caption{Ablation of the proposed modules on ImageNet-1K.}
    % \vspace{-0.5em}
    \label{tab:ablation_in1k}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
                                    & ResNet-50   & ViT-B       \\ \hline
    \gray{SimMIM}                   & \gray{78.2} & \gray{83.1} \\
    $\mathcal{L}_{spa}$             & 78.4        & 83.2      \\
    $+\mathcal{L}_{freq}$           & 78.6        & 83.4      \\
    $+\mathcal{L}_{freq} + T (l^*)$ & \bf{78.8}   & \bf{83.5} \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/tab_in1k_vit_extend.tex <==
%%% old version for ICLR'2023
\begin{table}[t]
    \vspace{-0.5em}
    \setlength{\tabcolsep}{1.1mm}
    \centering
    \caption{ImageNet-1K fine-tuning (FT) top-1 accuracy (\%) with ResNet (R) and ViT of various model scales. We adopt the 100-epoch fine-tuning protocols for both architectures.}
    \label{tab:in1k_vit_extend}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|ccc|ccc}
    \toprule
Methods                    & Supervision  & ViT-S       & ViT-B       & ViT-L       & R-50        & R-101       & R-152       \\ \hline
\gray{Sup.}                & \gray{Label} & \gray{79.9} & \gray{81.8} & \gray{82.6} & \gray{78.9} & \gray{79.8} & \gray{80.7} \\
MoCoV3                     & CL           & 81.4        & 83.2        & 84.1        & \bf{79.0}   & 80.1        & -           \\ \hline
MAE                        & RGB          & -           & 83.6        & 85.9        & 77.2        & 79.0        & 79.8        \\
SimMIM                     & RGB          & 81.7        & 83.8        & 85.6        & 78.1        & 79.9        & 80.4        \\
\rowcolor{gray94}A$^2$MIM  & RGB          & \ul{82.2}   & \ul{84.2}   & \ul{86.1}   & \ul{78.9}   & \ul{80.3}   & \ul{80.9}   \\
\rowcolor{gray94}A$^2$MIM+ & HoG          & \bf{82.4}   & \bf{84.5}   & \bf{86.2}   & \bf{79.0}   & \bf{80.4}   & \bf{81.0}   \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1.25em}
\end{table}


% %%% full version of CNNs
% \begin{table}[t]
%     \vspace{-0.5em}
%     \setlength{\tabcolsep}{0.8mm}
%     \centering
%     \caption{ImageNet-1K fine-tuning (FT) top-1 accuracy (\%) with ResNet (R) and ViT of various model scales. We adopt the 100-epoch fine-tuning protocols for both architectures.}
%     \label{tab:in1k_vit_extend}
% \resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{l|cc|ccccc >{\columncolor{gray94}}c >{\columncolor{gray94}}c}
%     \toprule
%     Methods     & \#Para. & FLOPs & \gray{Sup.}  & MoCoV3    & MAE  & SimMIM & \gray{SparK} & A$^2$MIM  & A$^2$MIM+ \\
%     Supervision & (M)     & (G)   & \gray{Label} & CL        & RGB  & RGB    & \gray{RGB}   & RGB       & HoG       \\ \hline
%     ResNet-50   & 25.6    & 4.1   & \gray{79.8}  & 80.1      & 79.0 & 79.9   & \gray{80.6}  & \ul{80.4} & \bf{80.5} \\
%     ResNet-101  & 44.5    & 7.9   & \gray{81.3}  & 81.6      & 80.3 & 81.3   & \gray{82.2}  & \ul{81.9} & \bf{82.0} \\
%     ResNet-152  & 60.2    & 11.6  & \gray{81.8}  & 82.0      & 80.9 & 81.9   & \gray{82.7}  & \ul{82.3} & \bf{82.5} \\ \hline
%     ConvNeXt-T  & 28.6    & 5.0   & \gray{82.1}  & 82.3      & 81.6 & 82.1   & \gray{82.7}  & \ul{82.4} & \bf{82.6} \\
%     ConvNeXt-S  & 50.2    & 8.8   & \gray{83.1}  & 83.3      & 82.5 & 83.2   & \gray{84.1}  & \ul{83.8} & \bf{83.9} \\
%     ConvNeXt-B  & 88.6    & 15.4  & \gray{83.5}  & 83.7      & 82.9 & 83.6   & \gray{84.8}  & \ul{84.3} & \bf{84.4} \\ \hline
%     ViT-S       & 22.1    & 4.6   & \gray{79.9}  & 81.4      & 81.6 & 81.7   & -            & \ul{82.2} & \bf{82.4} \\
%     ViT-B       & 86.6    & 17.5  & \gray{81.8}  & 83.2      & 83.6 & 83.8   & -            & \ul{84.2} & \bf{84.5} \\
%     ViT-L       & 304     & 44.8  & \gray{82.6}  & 84.1      & 85.9 & 85.6   & -            & \ul{86.1} & \bf{86.2} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{-1.25em}
% \end{table}

